Fine-tuning Pre-trained Language Models for Few-shot Intent Detection: Supervised Pre-training and Isotropization

It is challenging to train a good intent classifier for a task-oriented dialogue system with only a few annotations. Recent studies have shown that fine-tuning pre-trained language models with a small amount of labeled utterances from public benchmarks in a supervised manner is extremely helpful. However, we find that supervised pre-training yields an anisotropic feature space, which may suppress the expressive power of the semantic representations. Inspired by recent research in isotropization, we propose to improve supervised pre-training by regularizing the feature space towards isotropy. We propose two regularizers based on contrastive learning and correlation matrix respectively, and demonstrate their effectiveness through extensive experiments. Our main finding is that it is promising to regularize supervised pre-training with isotropization to further improve the performance of few-shot intent detection. The source code can be found at https://github.com/fanolabs/isoIntentBert-main.

==> sections/analysis.tex <==
\section{Analysis}
\textbf{CL-Reg and Cor-Reg render the feature space more isotropic.} 
\input{tables/table_analysis_isotropyChange_English}
% \input{tables/table_analysis_isotropyChange_crossLingual}
As shown in Table~\ref{table_analysis_isotropy_change_English}, both regularizers manage to make the feature space more isotropic, compared to IntentBERT-ReImp where only supervised pre-training is employed. In addition, Cor-Reg achieves similar or better isotropy compared to CL-Reg, which is consistent with Cor-Reg's relative superiority in performance. Interestingly, when the two regularizers are adopted simultaneously, the isotropy is not further improved, but a better performance is observed.

As for cross-lingual scenario, we summarize the results in Table~\ref{table_analysis_isotropy_change_CrossLingual}. Similar to experiments in English, both regularizers render the semantic space more isotropic. However, CL-Reg is less effective than Cor-Reg, for example, in Thai and Chinese, although they achieve similar performance. This observation indicates that the effectiveness of CL-Reg may not be ascribed to the improved isotropy for some target languages, which partially explains its complementarity with Cor-Reg. As shown in the table, when they are employed simultaneously, both the isotropy and the performance are improved.

% \noindent
\textbf{Moderate isotropy is helpful.}
To investigate the relation of isotropy and performance, we tune the weight on Cor-Reg to yield different degrees of isotropy and examine the corresponding performance. As shown in Fig.~\ref{figure: acc_iso_curve}, a common pattern is observed for most datasets -- the best performance is achieved only when the isotropy is moderate. 
% The accuracy-isotropy curve tends to rise when isotropy is low and drops when isotropy reaches near $1.0$, a perfect isotropy.
This observation indicates an appropriate trade-off between supervised pre-training and the isotropization that is achieved by the proposed method. 
% The measurement of isotropy is described in the appendix.
\input{figures/figure_acc_iso_curve}

\subsection{Correlation matrix is advantageous over covariance matrix}
In the design of Cor-Reg, correlation matrix, rather than covariance is employed to characterize isotropy, although the latter contains more information -- variance. We argue that the design choice is advantageous. We conduct experiments using covariance matrix. Particularly, the non-diagonal elements are pushed towards $0$, while the diagonal elements towards $1$, $0.5$ and the mean value, respectively, which are denoted by Cov-Reg-1, Cov-Reg-0.5 and Cov-Reg-mean in Table~\ref{table: analysis, coefficient matrix, or covariance matrix}. As shown in Table~\ref{table: analysis, coefficient matrix, or covariance matrix}, all these configurations under-perform Cor-Reg.
%  -- it avoids determining the variance value to optimize towards, which is difficult, while yields a superior performance. 
% because Cor-reg allows the learned knowledge to be encoded in elongations toward different directions.
\input{tables/table_analysis_correlation_covariance}

%\noindent
\textbf{The proposed methods are complementary with batch normalization.} Batch normalization~\cite{ICML-2015-IoffeS} is an off-the-shelf effective method to mitigate the anisotropy via normalizing each dimension into a scalar with zero mean and unit variance. 
% The normalization is implemented by learning a linear transformation for each dimension during training. 
As shown in Table~\ref{table: analysis, batch normalization}, our methods outperform batch normalization, and combining them yields even better performance.
%More importantly, their benefits are complementary.
% when they are adopted simultaneously, we observe the best performance.
\input{tables/table_analysis_batchNorm} 

==> tables/table_analysis_batchNorm_backup.tex <==
\begin{table}[h]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\centering
\small
\begin{tabular}{lcc}
\toprule
Method & BANKING77 & Val. \\
\midrule
SPT+BatchNorm  & 82.38\tiny{(.38)} &  94.78\tiny{(.24)}  \\
\midrule
SPT+CL-Reg  & 83.45\tiny{(.35)} & 94.43\tiny{(.22)} \\
\hspace{0.55cm}+BatchNorm  & \textbf{84.18\tiny{(.28)}} & \textbf{95.10\tiny{(.20)}} \\
\midrule
SPT+Cor-Reg  & 83.94\tiny{(.45)} & 95.02\tiny{(.22)} \\
\hspace{0.55cm}+BatchNorm  & \textbf{84.67\tiny{(.51)}} & \textbf{95.22\tiny{(.18)}} \\
\midrule
SPT+Cor-Reg+CL-Reg & 85.21\tiny{(.58)} & 95.41\tiny{(.25)} \\\hspace{0.55cm}+BatchNorm  & \textbf{85.64\tiny{(.41)}} & \textbf{95.57\tiny{(.25)}} \\
%\midrule
%SPT+CL-Reg+Cor-Reg+BatchNorm  &  85.21\tiny{$~\pm$.58} & 95.41\tiny{$~\pm$.25} \\
\bottomrule
\end{tabular}
% \caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper. $\ssymbol{2}$ represents models that employ Roberta.}
\caption{
%The complementarity of the proposed methods and batch normalization. 
Effect of combining batch normalization and our method. The experiments are conducted with BERT and evaluated on $5$-way $2$-shot tasks. SPT denotes supervised pre-training. BatchNorm denotes batch normalization.}
\label{table: analysis, batch normalization}
\end{table}
